Decomposition with Monotone B-splines: Fitting and Testing

A univariate continuous function can always be decomposed as the sum of a non-increasing function and a non-decreasing one. Based on this property, we propose a non-parametric regression method that combines two spline-fitted monotone curves. We demonstrate by extensive simulations that, compared to standard spline-fitting methods, the proposed approach is particularly advantageous in high-noise scenarios. Several theoretical guarantees are established for the proposed approach. Additionally, we present statistics to test the monotonicity of a function based on monotone decomposition, which can better control Type I error and achieve comparable (if not always higher) power compared to existing methods. Finally, we apply the proposed fitting and testing approaches to analyze the single-cell pseudotime trajectory datasets, identifying significant biological insights for non-monotonically expressed genes through Gene Ontology enrichment analysis. The source code implementing the methodology and producing all results is accessible at https://github.com/szcf-weiya/MonotoneDecomposition.jl.

==> figs/2022-02-06T10_07_11+08_00.tex <==
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{curve} & \multirow{2}{*}{noise}
&\multicolumn{2}{c}{MSFE}&\multicolumn{2}{c}{MSPE}\tabularnewline
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&&SS&MBSS&SS&MBSS\tabularnewline
\midrule
\multirow{3}{*}{$x^2$}&0.2& 1.92e+00 (1.7e-01)& 1.93e+00 (1.7e-01)& \textbf{1.33e+00} (4.3e-01)& 1.37e+00 (4.1e-01)\tabularnewline
&1.0& 9.80e+00 (8.1e-01)& 9.81e+00 (8.1e-01)& \textbf{6.13e+00} (2.4e+00)& 6.15e+00 (2.3e+00)\tabularnewline
&2.0& 1.95e+01 (1.5e+00)& 1.96e+01 (1.5e+00)& 1.20e+01 (4.2e+00)& \textbf{1.16e+01} (3.9e+00)\tabularnewline
\midrule
\multirow{3}{*}{$x^3$}&0.2& 1.92e+00 (1.5e-01)& 1.93e+00 (1.5e-01)& 1.56e+00 (4.5e-01)& \textbf{1.54e+00} (4.4e-01)\tabularnewline
&1.0& 9.59e+00 (8.0e-01)& 9.61e+00 (7.9e-01)& 6.86e+00 (2.5e+00)& \textbf{6.61e+00} (2.4e+00)\tabularnewline
&2.0& 1.94e+01 (2.0e+00)& 1.95e+01 (1.9e+00)& 1.24e+01 (6.5e+00)& \textbf{1.16e+01} (5.8e+00)\tabularnewline
\midrule
\multirow{3}{*}{$\exp(x)$}&0.2& 1.90e+00 (1.8e-01)& 1.90e+00 (1.7e-01)& \textbf{1.47e+00} (6.2e-01)& 1.48e+00 (6.0e-01)\tabularnewline
&1.0& 9.61e+00 (9.0e-01)& 9.62e+00 (8.9e-01)& 5.98e+00 (2.4e+00)& \textbf{5.79e+00} (2.3e+00)\tabularnewline
&2.0& 1.91e+01 (1.6e+00)& 1.92e+01 (1.6e+00)& 1.23e+01 (5.8e+00)& \textbf{1.17e+01} (5.1e+00)\tabularnewline
\midrule
\multirow{3}{*}{sigmoid}&0.2& 1.91e+00 (1.3e-01)& 1.91e+00 (1.3e-01)& 1.47e+00 (5.2e-01)& \textbf{1.45e+00} (5.1e-01)\tabularnewline
&1.0& 9.55e+00 (6.9e-01)& 9.57e+00 (6.8e-01)& 6.31e+00 (3.1e+00)& \textbf{6.16e+00} (2.9e+00)\tabularnewline
&2.0& 1.93e+01 (1.8e+00)& 1.93e+01 (1.7e+00)& 1.12e+01 (6.8e+00)& \textbf{1.06e+01} (6.2e+00)\tabularnewline
\midrule
\multirow{3}{*}{SE-1}&0.2& 1.92e+00 (1.6e-01)& 1.92e+00 (1.6e-01)& \textbf{1.41e+00} (5.4e-01)& 1.43e+00 (5.3e-01)\tabularnewline
&1.0& 9.69e+00 (6.8e-01)& 9.71e+00 (6.8e-01)& 5.99e+00 (2.4e+00)& \textbf{5.93e+00} (2.2e+00)\tabularnewline
&2.0& 1.95e+01 (1.7e+00)& 1.95e+01 (1.5e+00)& 1.24e+01 (6.3e+00)& \textbf{1.17e+01} (5.6e+00)\tabularnewline
\midrule
\multirow{3}{*}{SE-0.1}&0.2& 1.65e+00 (1.6e-01)& 1.67e+00 (1.7e-01)& \textbf{3.04e+00} (4.2e-01)& 3.09e+00 (4.4e-01)\tabularnewline
&1.0& 9.00e+00 (9.2e-01)& 9.07e+00 (9.3e-01)& \textbf{1.21e+01} (2.3e+00)& 1.22e+01 (2.3e+00)\tabularnewline
&2.0& 1.90e+01 (2.1e+00)& 1.91e+01 (2.0e+00)& 2.18e+01 (4.8e+00)& \textbf{2.13e+01} (4.3e+00)\tabularnewline
\midrule
\multirow{3}{*}{Mat12-1}&0.2& 1.97e+00 (2.9e-01)& 2.02e+00 (2.8e-01)& \textbf{4.79e+00} (3.7e-01)& 4.81e+00 (3.8e-01)\tabularnewline
&1.0& 9.64e+00 (8.5e-01)& 9.67e+00 (8.2e-01)& 1.08e+01 (1.7e+00)& \textbf{1.07e+01} (1.6e+00)\tabularnewline
&2.0& 1.93e+01 (1.6e+00)& 1.93e+01 (1.6e+00)& 1.64e+01 (4.0e+00)& \textbf{1.60e+01} (3.7e+00)\tabularnewline
\midrule
\multirow{3}{*}{Mat12-0.1}&0.2& 3.00e+00 (5.2e-01)& 3.16e+00 (4.8e-01)& \textbf{1.06e+01} (7.0e-01)& 1.08e+01 (6.8e-01)\tabularnewline
&1.0& 9.94e+00 (1.3e+00)& 1.01e+01 (1.3e+00)& 1.90e+01 (2.1e+00)& \textbf{1.90e+01} (2.0e+00)\tabularnewline
&2.0& 1.96e+01 (2.0e+00)& 1.98e+01 (2.0e+00)& 2.64e+01 (4.1e+00)& \textbf{2.61e+01} (3.7e+00)\tabularnewline
\midrule
\multirow{3}{*}{Mat32-1}&0.2& 1.87e+00 (1.7e-01)& 1.88e+00 (1.6e-01)& 2.03e+00 (5.3e-01)& \textbf{2.01e+00} (4.9e-01)\tabularnewline
&1.0& 9.53e+00 (8.3e-01)& 9.54e+00 (8.2e-01)& 7.77e+00 (2.7e+00)& \textbf{7.63e+00} (2.5e+00)\tabularnewline
&2.0& 1.95e+01 (1.5e+00)& 1.95e+01 (1.5e+00)& 1.22e+01 (4.6e+00)& \textbf{1.19e+01} (4.3e+00)\tabularnewline
\midrule
\multirow{3}{*}{Mat32-0.1}&0.2& 1.63e+00 (2.3e-01)& 1.70e+00 (2.3e-01)& \textbf{4.56e+00} (3.9e-01)& 4.62e+00 (4.3e-01)\tabularnewline
&1.0& 9.20e+00 (1.1e+00)& 9.30e+00 (1.1e+00)& 1.48e+01 (2.2e+00)& \textbf{1.47e+01} (2.1e+00)\tabularnewline
&2.0& 1.92e+01 (1.8e+00)& 1.93e+01 (1.8e+00)& 2.36e+01 (4.0e+00)& \textbf{2.32e+01} (3.8e+00)\tabularnewline
\midrule
\multirow{3}{*}{RQ-0.1-0.5}&0.2& 1.60e+00 (2.1e-01)& 1.65e+00 (2.0e-01)& \textbf{3.65e+00} (4.1e-01)& 3.67e+00 (4.2e-01)\tabularnewline
&1.0& 9.36e+00 (8.8e-01)& 9.42e+00 (8.7e-01)& 1.26e+01 (2.3e+00)& \textbf{1.25e+01} (2.2e+00)\tabularnewline
&2.0& 1.90e+01 (1.9e+00)& 1.91e+01 (1.8e+00)& 2.06e+01 (4.9e+00)& \textbf{2.03e+01} (4.6e+00)\tabularnewline
\midrule
\multirow{3}{*}{Periodic-0.1-4}&0.2& 1.51e+00 (2.0e-01)& 1.54e+00 (2.1e-01)& \textbf{3.79e+00} (4.5e-01)& 3.84e+00 (4.4e-01)\tabularnewline
&1.0& 8.94e+00 (9.7e-01)& 9.06e+00 (9.2e-01)& 1.47e+01 (2.0e+00)& \textbf{1.47e+01} (2.0e+00)\tabularnewline
&2.0& 1.91e+01 (2.5e+00)& 1.92e+01 (2.3e+00)& 2.58e+01 (5.4e+00)& \textbf{2.54e+01} (4.9e+00)\tabularnewline
\bottomrule
\end{tabular}


==> figs/2022-02-27T01_55_53+08_00.tex <==
\begin{tabular}{cccccccll}
\toprule
\multirow{2}{*}{curve} & \multirow{2}{*}{$\sigma$}& \multirow{2}{*}{SNR}&\multicolumn{2}{c}{MSFE}&\multicolumn{2}{c}{MSPE}& \multirow{2}{*}{p-value}& \multirow{2}{*}{prop.}\tabularnewline
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
&&&SmoothSpline&MonoDecomp&SmoothSpline&MonoDecomp\tabularnewline
\midrule
\multirow{6}{*}{$x^2$}&0.1& 1.08e+01 (6.5e-01)& 9.02e-03 (4.1e-04)& 9.53e-03 (3.9e-04)& \textbf{7.94e-04} (1.4e-04)& 1.16e-03 (1.4e-04)& 1.07e-04 (***)& 0.15\tabularnewline
&0.2& 2.93e+00 (3.0e-01)& 3.57e-02 (1.6e-03)& 3.61e-02 (1.5e-03)& \textbf{2.91e-03} (6.9e-04)& 3.04e-03 (6.1e-04)& 2.24e-01& 0.3\tabularnewline
&0.5& 5.36e-01 (3.1e-02)& 2.17e-01 (8.2e-03)& 2.20e-01 (7.9e-03)& 1.33e-02 (2.3e-03)& \textbf{1.22e-02} (1.9e-03)& 1.13e-01& 0.55\tabularnewline
&1.0& 1.46e-01 (1.8e-02)& 9.57e-01 (2.6e-02)& 9.62e-01 (2.7e-02)& \textbf{3.65e-02} (4.5e-03)& 4.03e-02 (5.1e-03)& 2.91e-02 (*)& 0.5\tabularnewline
&1.5& 1.33e-01 (2.4e-02)& 2.12e+00 (6.8e-02)& 2.19e+00 (7.8e-02)& 1.38e-01 (2.8e-02)& \textbf{1.10e-01} (2.1e-02)& 2.73e-02 (*)& 0.4\tabularnewline
&2.0& 6.67e-02 (1.5e-02)& 3.93e+00 (1.2e-01)& 3.98e+00 (1.3e-01)& 1.54e-01 (2.9e-02)& \textbf{1.36e-01} (2.0e-02)& 9.23e-02 (.)& 0.65\tabularnewline
\midrule
\multirow{6}{*}{$x^3$}&0.1& 1.89e+01 (8.3e-01)& 8.57e-03 (3.0e-04)& 9.88e-03 (3.5e-04)& \textbf{7.27e-04} (7.1e-05)& 1.60e-03 (1.5e-04)& 1.76e-10 (***)& 0.05\tabularnewline
&0.2& 4.13e+00 (1.1e-01)& 3.73e-02 (1.3e-03)& 3.86e-02 (1.3e-03)& \textbf{2.52e-03} (3.6e-04)& 3.31e-03 (2.9e-04)& 4.58e-04 (***)& 0.3\tabularnewline
&0.5& 7.09e-01 (5.6e-02)& 2.34e-01 (8.4e-03)& 2.38e-01 (7.4e-03)& 1.85e-02 (2.6e-03)& \textbf{1.66e-02} (1.9e-03)& 7.15e-02 (.)& 0.6\tabularnewline
&1.0& 2.95e-01 (6.5e-02)& 9.41e-01 (5.5e-02)& 9.61e-01 (5.3e-02)& 6.16e-02 (1.3e-02)& \textbf{5.29e-02} (1.1e-02)& 1.52e-01& 0.6\tabularnewline
&1.5& 1.18e-01 (1.9e-02)& 2.14e+00 (9.4e-02)& 2.15e+00 (9.4e-02)& 8.07e-02 (1.2e-02)& \textbf{7.37e-02} (9.1e-03)& 4.33e-02 (*)& 0.65\tabularnewline
&2.0& 8.84e-02 (1.8e-02)& 3.82e+00 (1.5e-01)& 3.86e+00 (1.5e-01)& 1.55e-01 (2.9e-02)& \textbf{1.22e-01} (2.4e-02)& 4.38e-02 (*)& 0.8\tabularnewline
\midrule
\multirow{6}{*}{$\exp(x)$}&0.1& 4.63e+01 (1.4e+00)& 9.75e-03 (2.6e-04)& 1.03e-02 (2.6e-04)& \textbf{5.50e-04} (8.3e-05)& 1.13e-03 (1.3e-04)& 2.29e-08 (***)& 0.1\tabularnewline
&0.2& 1.22e+01 (4.1e-01)& 3.69e-02 (1.3e-03)& 3.75e-02 (1.3e-03)& \textbf{1.79e-03} (2.2e-04)& 2.26e-03 (2.7e-04)& 5.51e-03 (**)& 0.35\tabularnewline
&0.5& 2.26e+00 (1.6e-01)& 2.28e-01 (1.0e-02)& 2.30e-01 (9.5e-03)& 1.73e-02 (4.0e-03)& \textbf{1.60e-02} (2.9e-03)& 1.65e-01& 0.4\tabularnewline
&1.0& 5.42e-01 (3.8e-02)& 9.13e-01 (4.1e-02)& 9.19e-01 (4.1e-02)& 4.11e-02 (5.2e-03)& \textbf{3.95e-02} (4.6e-03)& 2.76e-01& 0.55\tabularnewline
&1.5& 2.65e-01 (4.2e-02)& 2.22e+00 (9.7e-02)& 2.24e+00 (9.3e-02)& 1.00e-01 (3.1e-02)& \textbf{8.70e-02} (2.2e-02)& 2.68e-01& 0.4\tabularnewline
&2.0& 1.69e-01 (1.7e-02)& 3.74e+00 (7.7e-02)& 3.76e+00 (7.9e-02)& 1.15e-01 (2.1e-02)& \textbf{1.14e-01} (1.9e-02)& 4.60e-01& 0.4\tabularnewline
\midrule
\multirow{6}{*}{sigmoid}&0.1& 1.71e+01 (5.1e-01)& 9.25e-03 (2.6e-04)& 9.24e-03 (2.6e-04)& \textbf{5.58e-04} (6.1e-05)& 5.59e-04 (5.8e-05)& 4.86e-01& 0.45\tabularnewline
&0.2& 4.42e+00 (2.8e-01)& 3.65e-02 (1.5e-03)& 3.65e-02 (1.5e-03)& \textbf{2.13e-03} (2.2e-04)& 2.17e-03 (2.3e-04)& 3.02e-01& 0.65\tabularnewline
&0.5& 6.98e-01 (6.7e-02)& 2.45e-01 (7.5e-03)& 2.46e-01 (7.4e-03)& 1.65e-02 (3.1e-03)& \textbf{1.57e-02} (2.5e-03)& 2.80e-01& 0.5\tabularnewline
&1.0& 2.28e-01 (3.1e-02)& 9.48e-01 (3.2e-02)& 9.53e-01 (3.1e-02)& 4.41e-02 (1.3e-02)& \textbf{4.33e-02} (1.1e-02)& 4.22e-01& 0.35\tabularnewline
&1.5& 1.19e-01 (1.6e-02)& 2.27e+00 (6.1e-02)& 2.28e+00 (6.3e-02)& 7.37e-02 (1.6e-02)& \textbf{6.62e-02} (1.5e-02)& 3.92e-02 (*)& 0.45\tabularnewline
&2.0& 8.16e-02 (1.7e-02)& 4.09e+00 (1.4e-01)& 4.13e+00 (1.4e-01)& 1.54e-01 (2.9e-02)& \textbf{1.47e-01} (2.8e-02)& 1.89e-01& 0.6\tabularnewline
\midrule
\multirow{6}{*}{SE-1}&0.1& 2.00e+01 (5.3e+00)& 9.73e-03 (3.1e-04)& 1.00e-02 (3.1e-04)& \textbf{5.48e-04} (7.5e-05)& 5.72e-04 (7.1e-05)& 2.46e-01& 0.35\tabularnewline
&0.2& 1.16e+01 (3.1e+00)& 3.69e-02 (1.2e-03)& 3.73e-02 (1.2e-03)& \textbf{2.27e-03} (3.6e-04)& 2.50e-03 (4.3e-04)& 8.55e-02 (.)& 0.45\tabularnewline
&0.5& 1.24e+00 (3.0e-01)& 2.20e-01 (8.9e-03)& 2.20e-01 (8.7e-03)& 1.56e-02 (2.8e-03)& \textbf{1.54e-02} (2.7e-03)& 3.82e-01& 0.45\tabularnewline
&1.0& 3.38e-01 (1.2e-01)& 9.52e-01 (4.2e-02)& 9.58e-01 (4.2e-02)& 3.93e-02 (7.1e-03)& \textbf{3.80e-02} (6.5e-03)& 1.79e-01& 0.5\tabularnewline
&1.5& 2.53e-01 (6.4e-02)& 2.14e+00 (6.5e-02)& 2.16e+00 (6.3e-02)& 1.17e-01 (2.2e-02)& \textbf{9.39e-02} (1.6e-02)& 4.21e-03 (**)& 0.5\tabularnewline
&2.0& 1.42e-01 (2.6e-02)& 3.86e+00 (1.4e-01)& 3.93e+00 (1.3e-01)& 1.34e-01 (2.2e-02)& \textbf{1.15e-01} (1.9e-02)& 5.37e-02 (.)& 0.85\tabularnewline
\midrule
\multirow{6}{*}{SE-0.1}&0.1& 1.48e+02 (1.4e+01)& 5.74e-03 (2.4e-04)& 6.39e-03 (3.1e-04)& \textbf{3.10e-03} (1.8e-04)& 3.34e-03 (2.1e-04)& 5.01e-04 (***)& 0.35\tabularnewline
&0.2& 3.77e+01 (5.8e+00)& 2.73e-02 (1.6e-03)& 2.96e-02 (1.7e-03)& \textbf{1.04e-02} (6.0e-04)& 1.08e-02 (6.4e-04)& 8.50e-02 (.)& 0.35\tabularnewline
&0.5& 4.41e+00 (4.9e-01)& 1.92e-01 (9.4e-03)& 1.98e-01 (8.6e-03)& \textbf{4.89e-02} (3.6e-03)& 4.95e-02 (3.7e-03)& 2.92e-01& 0.4\tabularnewline
&1.0& 1.14e+00 (1.3e-01)& 8.70e-01 (3.2e-02)& 8.95e-01 (3.5e-02)& \textbf{1.48e-01} (7.5e-03)& 1.55e-01 (8.5e-03)& 4.30e-02 (*)& 0.3\tabularnewline
&1.5& 6.51e-01 (6.0e-02)& 1.83e+00 (7.7e-02)& 1.87e+00 (7.6e-02)& 3.24e-01 (3.1e-02)& \textbf{3.19e-01} (2.8e-02)& 2.39e-01& 0.35\tabularnewline
&2.0& 3.94e-01 (4.0e-02)& 3.57e+00 (1.3e-01)& 3.67e+00 (1.4e-01)& 4.80e-01 (3.9e-02)& \textbf{4.73e-01} (3.9e-02)& 3.32e-01& 0.7\tabularnewline
\midrule
\multirow{6}{*}{Mat12-1}&0.1& 2.80e+01 (4.5e+00)& 1.53e-02 (1.2e-03)& 1.77e-02 (1.3e-03)& \textbf{1.40e-02} (5.8e-04)& 1.51e-02 (7.3e-04)& 1.27e-03 (**)& 0.05\tabularnewline
&0.2& 1.10e+01 (1.7e+00)& 3.96e-02 (3.3e-03)& 4.43e-02 (3.1e-03)& \textbf{2.55e-02} (1.3e-03)& 2.70e-02 (1.2e-03)& 2.86e-02 (*)& 0.25\tabularnewline
&0.5& 2.30e+00 (3.2e-01)& 2.25e-01 (1.1e-02)& 2.33e-01 (1.1e-02)& 6.26e-02 (2.8e-03)& \textbf{6.22e-02} (2.6e-03)& 2.78e-01& 0.6\tabularnewline
&1.0& 4.90e-01 (5.9e-02)& 9.88e-01 (3.3e-02)& 1.00e+00 (3.5e-02)& 1.27e-01 (6.1e-03)& \textbf{1.22e-01} (6.1e-03)& 5.20e-02 (.)& 0.65\tabularnewline
&1.5& 4.14e-01 (8.8e-02)& 2.08e+00 (6.3e-02)& 2.13e+00 (6.0e-02)& 2.10e-01 (1.9e-02)& \textbf{1.87e-01} (1.8e-02)& 3.72e-02 (*)& 0.55\tabularnewline
&2.0& 1.20e-01 (2.0e-02)& 3.84e+00 (1.4e-01)& 3.87e+00 (1.4e-01)& \textbf{2.35e-01} (1.6e-02)& 2.36e-01 (1.7e-02)& 4.22e-01& 0.75\tabularnewline
\midrule
\multirow{6}{*}{Mat12-0.1}&0.1& 1.25e+01 (1.4e+00)& 7.31e-02 (5.3e-03)& 8.81e-02 (5.9e-03)& \textbf{1.02e-01} (3.9e-03)& 1.13e-01 (5.0e-03)& 5.43e-07 (***)& 0.05\tabularnewline
&0.2& 1.10e+01 (1.4e+00)& 9.20e-02 (7.2e-03)& 1.11e-01 (7.0e-03)& \textbf{1.17e-01} (2.9e-03)& 1.27e-01 (3.6e-03)& 5.75e-07 (***)& 0.15\tabularnewline
&0.5& 3.77e+00 (4.3e-01)& 2.46e-01 (1.4e-02)& 3.09e-01 (2.2e-02)& \textbf{1.95e-01} (7.4e-03)& 2.15e-01 (1.0e-02)& 2.95e-02 (*)& 0.4\tabularnewline
&1.0& 1.15e+00 (1.3e-01)& 9.44e-01 (5.1e-02)& 9.96e-01 (5.0e-02)& 3.73e-01 (1.2e-02)& \textbf{3.72e-01} (1.4e-02)& 4.77e-01& 0.3\tabularnewline
&1.5& 5.07e-01 (7.1e-02)& 2.29e+00 (9.7e-02)& 2.39e+00 (8.9e-02)& \textbf{5.03e-01} (2.6e-02)& 5.15e-01 (2.6e-02)& 1.59e-01& 0.5\tabularnewline
&2.0& 1.92e-01 (3.6e-02)& 3.97e+00 (1.7e-01)& 4.04e+00 (1.7e-01)& \textbf{6.82e-01} (4.5e-02)& 6.82e-01 (4.5e-02)& 4.82e-01& 0.5\tabularnewline
\midrule
\multirow{6}{*}{Mat32-1}&0.1& 4.10e+01 (8.8e+00)& 8.73e-03 (4.1e-04)& 8.97e-03 (3.9e-04)& \textbf{1.54e-03} (1.3e-04)& 1.56e-03 (1.4e-04)& 2.50e-01& 0.35\tabularnewline
&0.2& 9.75e+00 (2.5e+00)& 3.57e-02 (1.5e-03)& 3.68e-02 (1.3e-03)& 5.44e-03 (6.0e-04)& \textbf{5.25e-03} (3.5e-04)& 3.46e-01& 0.5\tabularnewline
&0.5& 1.58e+00 (4.0e-01)& 2.22e-01 (7.7e-03)& 2.26e-01 (7.9e-03)& \textbf{1.84e-02} (2.1e-03)& 1.84e-02 (2.4e-03)& 4.78e-01& 0.55\tabularnewline
&1.0& 5.57e-01 (1.3e-01)& 9.28e-01 (3.8e-02)& 9.40e-01 (3.8e-02)& \textbf{6.74e-02} (1.1e-02)& 6.90e-02 (8.4e-03)& 3.57e-01& 0.7\tabularnewline
&1.5& 2.76e-01 (6.3e-02)& 2.11e+00 (7.8e-02)& 2.15e+00 (8.0e-02)& 1.08e-01 (1.1e-02)& \textbf{9.45e-02} (8.4e-03)& 9.87e-03 (**)& 0.45\tabularnewline
&2.0& 2.08e-01 (5.0e-02)& 3.72e+00 (1.8e-01)& 3.75e+00 (1.8e-01)& 2.65e-01 (4.4e-02)& \textbf{2.29e-01} (3.9e-02)& 4.64e-03 (**)& 0.75\tabularnewline
\midrule
\multirow{6}{*}{Mat32-0.1}&0.1& 1.22e+02 (9.7e+00)& 8.09e-03 (3.8e-04)& 9.33e-03 (5.9e-04)& \textbf{8.76e-03} (3.1e-04)& 9.46e-03 (3.5e-04)& 9.01e-03 (**)& 0.25\tabularnewline
&0.2& 4.96e+01 (7.2e+00)& 2.42e-02 (1.6e-03)& 2.96e-02 (2.4e-03)& \textbf{2.24e-02} (9.4e-04)& 2.45e-02 (1.6e-03)& 4.06e-02 (*)& 0.1\tabularnewline
&0.5& 6.03e+00 (7.1e-01)& 1.87e-01 (1.1e-02)& 2.04e-01 (1.1e-02)& \textbf{7.67e-02} (3.5e-03)& 7.93e-02 (3.4e-03)& 6.68e-02 (.)& 0.4\tabularnewline
&1.0& 1.52e+00 (2.9e-01)& 8.51e-01 (5.0e-02)& 9.34e-01 (4.5e-02)& 2.26e-01 (1.5e-02)& \textbf{2.21e-01} (1.2e-02)& 2.76e-01& 0.45\tabularnewline
&1.5& 6.33e-01 (9.5e-02)& 1.91e+00 (7.9e-02)& 1.96e+00 (8.0e-02)& \textbf{3.28e-01} (2.0e-02)& 3.30e-01 (1.8e-02)& 4.21e-01& 0.55\tabularnewline
&2.0& 3.52e-01 (4.4e-02)& 3.76e+00 (1.2e-01)& 3.86e+00 (1.3e-01)& 5.76e-01 (4.7e-02)& \textbf{5.73e-01} (4.7e-02)& 4.30e-01& 0.55\tabularnewline
\midrule
\multirow{6}{*}{RQ-0.1-0.5}&0.1& 1.30e+02 (1.3e+01)& 6.21e-03 (3.1e-04)& 7.22e-03 (3.3e-04)& \textbf{3.79e-03} (2.1e-04)& 4.17e-03 (2.5e-04)& 2.53e-08 (***)& 0.1\tabularnewline
&0.2& 3.03e+01 (4.5e+00)& 2.46e-02 (1.4e-03)& 2.74e-02 (1.5e-03)& \textbf{1.26e-02} (7.1e-04)& 1.33e-02 (7.1e-04)& 8.32e-03 (**)& 0.3\tabularnewline
&0.5& 3.61e+00 (3.3e-01)& 1.95e-01 (8.6e-03)& 2.15e-01 (1.0e-02)& \textbf{5.91e-02} (3.4e-03)& 6.60e-02 (3.8e-03)& 3.92e-03 (**)& 0.2\tabularnewline
&1.0& 1.23e+00 (1.3e-01)& 8.19e-01 (3.7e-02)& 8.84e-01 (4.0e-02)& 1.85e-01 (1.5e-02)& \textbf{1.77e-01} (1.3e-02)& 8.94e-02 (.)& 0.4\tabularnewline
&1.5& 5.02e-01 (8.1e-02)& 2.10e+00 (8.7e-02)& 2.21e+00 (9.1e-02)& 3.25e-01 (4.4e-02)& \textbf{3.16e-01} (4.6e-02)& 2.54e-01& 0.6\tabularnewline
&2.0& 4.32e-01 (1.1e-01)& 3.49e+00 (1.8e-01)& 3.62e+00 (1.7e-01)& 5.56e-01 (8.4e-02)& \textbf{4.78e-01} (6.4e-02)& 2.55e-03 (**)& 0.6\tabularnewline
\midrule
\multirow{6}{*}{Periodic-0.1-4}&0.1& 1.89e+02 (2.3e+01)& 5.31e-03 (2.9e-04)& 6.02e-03 (3.4e-04)& \textbf{4.68e-03} (1.7e-04)& 4.86e-03 (2.0e-04)& 2.65e-02 (*)& 0.3\tabularnewline
&0.2& 4.18e+01 (6.4e+00)& 2.53e-02 (2.0e-03)& 2.80e-02 (2.0e-03)& \textbf{1.44e-02} (7.8e-04)& 1.52e-02 (7.2e-04)& 3.90e-02 (*)& 0.25\tabularnewline
&0.5& 6.00e+00 (5.9e-01)& 1.81e-01 (9.8e-03)& 1.98e-01 (1.0e-02)& \textbf{7.40e-02} (4.6e-03)& 8.09e-02 (5.2e-03)& 2.13e-05 (***)& 0.5\tabularnewline
&1.0& 1.43e+00 (1.3e-01)& 8.05e-01 (3.2e-02)& 8.56e-01 (3.6e-02)& 2.28e-01 (1.6e-02)& \textbf{2.22e-01} (1.7e-02)& 2.40e-01& 0.25\tabularnewline
&1.5& 5.99e-01 (8.4e-02)& 1.89e+00 (8.1e-02)& 1.96e+00 (8.0e-02)& \textbf{4.25e-01} (2.3e-02)& 4.46e-01 (2.8e-02)& 8.66e-02 (.)& 0.45\tabularnewline
&2.0& 3.19e-01 (5.2e-02)& 3.79e+00 (1.6e-01)& 3.90e+00 (1.5e-01)& \textbf{5.77e-01} (3.3e-02)& 5.80e-01 (3.7e-02)& 4.10e-01& 0.5\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_test/res_mono_test_bowman_sup.tex <==
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{a}&\multicolumn{3}{c}{$\sigma = 0.001$}&\multicolumn{3}{c}{$\sigma = 0.01$}&\multicolumn{3}{c}{$\sigma = 0.1$}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
&&n = 50&100&200&n = 50&100&200&n = 50&100&200\tabularnewline
\midrule
\midrule
\multirow{4}{*}{MD (CS) sup}&0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.02& 0.0& 0.01\tabularnewline
&0.15& 0.19& 0.28& 0.14& 0.31& 0.44& 0.28& 0.02& 0.01& 0.0\tabularnewline
&0.25& 0.99& 0.99& 1.0& 0.9& 0.99& 1.0& 0.15& 0.16& 0.22\tabularnewline
&0.45& 0.95& 0.96& 0.99& 0.95& 1.0& 1.0& 0.76& 0.89& 0.98\tabularnewline
\midrule
\multirow{4}{*}{MD (CS)}&0.0& 0.02& 0.05& 0.01& 0.02& 0.04& 0.02& 0.06& 0.05& 0.04\tabularnewline
&0.15& 0.25& 0.32& 0.18& 0.42& 0.51& 0.52& 0.1& 0.12& 0.04\tabularnewline
&0.25& 0.99& 0.99& 1.0& 0.91& 1.0& 1.0& 0.23& 0.24& 0.44\tabularnewline
&0.45& 0.95& 0.96& 0.99& 0.95& 1.0& 1.0& 0.86& 0.94& 0.99\tabularnewline
\midrule
\multirow{4}{*}{MD (SS) sup}&0.0& 0.0& 0.0& 0.0& 0.03& 0.0& 0.0& 0.03& 0.0& 0.01\tabularnewline
&0.15& 0.0& 0.0& 0.0& 0.04& 0.0& 0.0& 0.03& 0.0& 0.01\tabularnewline
&0.25& 0.0& 0.0& 0.99& 0.03& 0.0& 0.95& 0.04& 0.0& 0.0\tabularnewline
&0.45& 0.82& 1.0& 1.0& 0.97& 1.0& 1.0& 0.16& 0.59& 0.91\tabularnewline
\midrule
\multirow{4}{*}{MD (SS)}&0.0& 0.06& 0.1& 0.06& 0.08& 0.07& 0.1& 0.08& 0.05& 0.07\tabularnewline
&0.15& 0.03& 0.01& 0.04& 0.08& 0.0& 0.04& 0.08& 0.07& 0.05\tabularnewline
&0.25& 0.11& 0.11& 0.99& 0.06& 0.14& 0.97& 0.06& 0.03& 0.02\tabularnewline
&0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.23& 0.71& 1.0\tabularnewline
\midrule
\multirow{4}{*}{Meyer}&0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.02& 0.02& 0.0\tabularnewline
&0.15& 0.0& 0.0& 0.0& 0.1& 0.02& 0.06& 0.03& 0.04& 0.0\tabularnewline
&0.25& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.1& 0.34& 0.59\tabularnewline
&0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.64& 0.93& 1.0\tabularnewline
\midrule
\multirow{4}{*}{Ghosal}&0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&0.15& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&0.25& 0.0& 0.0& 1.0& 0.0& 0.0& 0.31& 0.0& 0.01& 0.0\tabularnewline
&0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.15& 0.76& 1.0\tabularnewline
\midrule
\multirow{4}{*}{Bowman}&0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.03& 0.01\tabularnewline
&0.15& 0.0& 0.0& 0.0& 0.0& 0.04& 0.03& 0.01& 0.02& 0.0\tabularnewline
&0.25& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.09& 0.17& 0.42\tabularnewline
&0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.36& 0.82& 1.0\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_test/res_mono_test_bowman_sup_NREP100_a295dc8_2023-09-11T09_07_44+08_00.tex <==
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Curves}&\multicolumn{3}{c}{$\sigma = 0.001$}&\multicolumn{3}{c}{$\sigma = 0.01$}&\multicolumn{3}{c}{$\sigma = 0.1$}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
&&n = 50&100&200&n = 50&100&200&n = 50&100&200\tabularnewline
\midrule
\midrule
\multirow{4}{*}{Meyer}&a = 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.02& 0.0& 0.0\tabularnewline
&a = 0.15& 0.0& 0.0& 0.0& 0.03& 0.04& 0.04& 0.02& 0.0& 0.03\tabularnewline
&a = 0.25& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.06& 0.22& 0.62\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.66& 0.9& 1.0\tabularnewline
\midrule
\multirow{4}{*}{Ghosal}&a = 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&a = 0.15& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&a = 0.25& 0.0& 0.0& 1.0& 0.0& 0.0& 0.33& 0.0& 0.0& 0.01\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.1& 0.67& 0.99\tabularnewline
\midrule
\multirow{4}{*}{Bowman}&a = 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.01& 0.02& 0.01& 0.0\tabularnewline
&a = 0.15& 0.0& 0.0& 0.0& 0.01& 0.01& 0.05& 0.01& 0.01& 0.04\tabularnewline
&a = 0.25& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.12& 0.17& 0.44\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.39& 0.76& 0.99\tabularnewline
\midrule
\multirow{4}{*}{MDCS}&a = 0.0& 0.03& 0.0& 0.01& 0.0& 0.0& 0.0& 0.01& 0.0& 0.0\tabularnewline
&a = 0.15& 0.04& 0.01& 0.0& 0.0& 0.01& 0.01& 0.0& 0.0& 0.0\tabularnewline
&a = 0.25& 0.7& 0.72& 0.66& 0.63& 0.83& 0.91& 0.0& 0.0& 0.0\tabularnewline
&a = 0.45& 0.68& 0.81& 0.74& 0.98& 0.92& 0.95& 0.02& 0.05& 0.16\tabularnewline
\midrule
\multirow{4}{*}{MDSS}&a = 0.0& 0.02& 0.05& 0.07& 0.02& 0.06& 0.03& 0.0& 0.05& 0.03\tabularnewline
&a = 0.15& 0.06& 0.05& 0.03& 0.08& 0.03& 0.04& 0.02& 0.04& 0.05\tabularnewline
&a = 0.25& 1.0& 1.0& 1.0& 0.98& 1.0& 1.0& 0.04& 0.07& 0.02\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.52& 0.85& 0.98\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_test/res_mono_test_bowman_sup_NREP100_a295dc8_2023-09-11T13_38_28+08_00.tex <==
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Curves}&\multicolumn{3}{c}{$\sigma = 0.001$}&\multicolumn{3}{c}{$\sigma = 0.01$}&\multicolumn{3}{c}{$\sigma = 0.1$}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
&&n = 50&100&200&n = 50&100&200&n = 50&100&200\tabularnewline
\midrule
\midrule
\multirow{4}{*}{\textcite{wangTestingMonotonicityConvexity2011}}&a = 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.01& 0.01& 0.01\tabularnewline
&a = 0.15& 0.0& 0.0& 0.0& 0.07& 0.04& 0.06& 0.03& 0.03& 0.01\tabularnewline
&a = 0.25& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.13& 0.24& 0.64\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.56& 0.95& 1.0\tabularnewline
\midrule
\multirow{4}{*}{\textcite{ghosalTestingMonotonicityRegression2000}}&a = 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&a = 0.15& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&a = 0.25& 0.0& 0.0& 1.0& 0.0& 0.0& 0.31& 0.0& 0.0& 0.0\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.06& 0.71& 0.99\tabularnewline
\midrule
\multirow{4}{*}{\textcite{bowmanTestingMonotonicityRegression1998}}&a = 0.0& 0.0& 0.0& 0.0& 0.02& 0.01& 0.0& 0.01& 0.01& 0.03\tabularnewline
&a = 0.15& 0.0& 0.0& 0.0& 0.0& 0.03& 0.0& 0.01& 0.02& 0.04\tabularnewline
&a = 0.25& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.09& 0.16& 0.44\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.3& 0.72& 0.98\tabularnewline
\midrule
\multirow{4}{*}{MDCS}&a = 0.0& 0.01& 0.0& 0.07& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&a = 0.15& 0.05& 0.02& 0.04& 0.01& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&a = 0.25& 0.97& 1.0& 1.0& 0.74& 0.92& 0.95& 0.0& 0.0& 0.0\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 0.99& 1.0& 1.0& 0.01& 0.08& 0.17\tabularnewline
\midrule
\multirow{4}{*}{MDSS}&a = 0.0& 0.02& 0.07& 0.06& 0.02& 0.08& 0.03& 0.02& 0.04& 0.04\tabularnewline
&a = 0.15& 0.05& 0.03& 0.05& 0.03& 0.06& 0.05& 0.02& 0.05& 0.06\tabularnewline
&a = 0.25& 0.99& 1.0& 1.0& 0.98& 1.0& 1.0& 0.03& 0.04& 0.03\tabularnewline
&a = 0.45& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.46& 0.82& 0.98\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_test/res_mono_test_ghosal_sup.tex <==
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{curve}&\multicolumn{3}{c}{$\sigma = 0.001$}&\multicolumn{3}{c}{$\sigma = 0.01$}&\multicolumn{3}{c}{$\sigma = 0.1$}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
&&n = 50&100&200&n = 50&100&200&n = 50&100&200\tabularnewline
\midrule
\midrule
\multirow{4}{*}{MD (CS) sup}&m1& 0.01& 0.0& 0.0& 0.02& 0.0& 0.0& 0.01& 0.0& 0.0\tabularnewline
&m2& 0.96& 1.0& 1.0& 0.97& 1.0& 1.0& 0.84& 0.99& 1.0\tabularnewline
&m3& 0.85& 0.92& 0.95& 0.95& 1.0& 1.0& 0.41& 0.59& 0.92\tabularnewline
&m4& 0.72& 0.84& 0.97& 0.7& 0.8& 0.94& 0.8& 0.96& 1.0\tabularnewline
\midrule
\multirow{4}{*}{MD (CS)}&m1& 0.08& 0.02& 0.06& 0.04& 0.03& 0.02& 0.04& 0.06& 0.04\tabularnewline
&m2& 0.96& 1.0& 1.0& 0.97& 1.0& 1.0& 0.91& 1.0& 1.0\tabularnewline
&m3& 0.85& 0.92& 0.95& 0.95& 1.0& 1.0& 0.62& 0.79& 0.99\tabularnewline
&m4& 0.73& 0.84& 0.97& 0.71& 0.8& 0.94& 0.81& 0.97& 1.0\tabularnewline
\midrule
\multirow{4}{*}{MD (SS) sup}&m1& 0.13& 0.01& 0.05& 0.16& 0.02& 0.03& 0.08& 0.02& 0.03\tabularnewline
&m2& 0.94& 1.0& 1.0& 0.95& 1.0& 0.99& 0.83& 1.0& 1.0\tabularnewline
&m3& 0.93& 1.0& 1.0& 0.86& 1.0& 0.99& 0.28& 0.56& 0.97\tabularnewline
&m4& 0.52& 0.99& 1.0& 0.41& 0.99& 0.99& 0.17& 0.9& 0.99\tabularnewline
\midrule
\multirow{4}{*}{MD (SS)}&m1& 0.21& 0.07& 0.1& 0.24& 0.09& 0.11& 0.11& 0.05& 0.11\tabularnewline
&m2& 0.98& 1.0& 1.0& 1.0& 1.0& 1.0& 0.9& 1.0& 1.0\tabularnewline
&m3& 0.95& 1.0& 1.0& 0.9& 1.0& 1.0& 0.41& 0.78& 1.0\tabularnewline
&m4& 0.64& 1.0& 1.0& 0.51& 0.99& 0.99& 0.38& 0.97& 0.99\tabularnewline
\midrule
\multirow{4}{*}{Meyer}&m1& 0.08& 0.04& 0.07& 0.08& 0.07& 0.02& 0.04& 0.03& 0.06\tabularnewline
&m2& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.17& 0.22& 0.46\tabularnewline
&m3& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.34& 0.64& 0.89\tabularnewline
&m4& 0.35& 0.63& 0.99& 0.34& 0.63& 0.99& 0.25& 0.34& 0.79\tabularnewline
\midrule
\multirow{4}{*}{Ghosal}&m1& 0.0& 0.02& 0.03& 0.0& 0.01& 0.0& 0.0& 0.01& 0.01\tabularnewline
&m2& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.26& 0.66& 0.94\tabularnewline
&m3& 0.95& 0.99& 1.0& 0.9& 1.0& 1.0& 0.15& 0.43& 0.84\tabularnewline
&m4& 0.05& 0.09& 0.53& 0.03& 0.17& 0.57& 0.0& 0.12& 0.34\tabularnewline
\midrule
\multirow{4}{*}{Bowman}&m1& 0.0& 0.01& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&m2& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&m3& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.92& 1.0& 1.0\tabularnewline
&m4& 0.0& 0.0& 0.0& 0.01& 0.01& 0.0& 0.35& 0.26& 0.18\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_test/res_mono_test_ghosal_sup_NREP100_a295dc8_2023-09-10T09_53_13+08_00.tex <==
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Curves}&\multicolumn{3}{c}{$\sigma = 0.001$}&\multicolumn{3}{c}{$\sigma = 0.01$}&\multicolumn{3}{c}{$\sigma = 0.1$}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
&&n = 50&100&200&n = 50&100&200&n = 50&100&200\tabularnewline
\midrule
\midrule
\multirow{4}{*}{\textcite{wangTestingMonotonicityConvexity2011}}&m1& 0.1& 0.04& 0.04& 0.06& 0.02& 0.06& 0.07& 0.07& 0.1\tabularnewline
&m2& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.09& 0.27& 0.45\tabularnewline
&m3& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.34& 0.56& 0.88\tabularnewline
&m4& 0.36& 0.57& 0.98& 0.39& 0.57& 0.98& 0.23& 0.38& 0.78\tabularnewline
\midrule
\multirow{4}{*}{\textcite{ghosalTestingMonotonicityRegression2000}}&m1& 0.01& 0.0& 0.01& 0.01& 0.04& 0.02& 0.02& 0.0& 0.01\tabularnewline
&m2& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.37& 0.7& 0.94\tabularnewline
&m3& 0.97& 1.0& 1.0& 0.94& 1.0& 1.0& 0.1& 0.33& 0.87\tabularnewline
&m4& 0.01& 0.19& 0.53& 0.02& 0.13& 0.53& 0.0& 0.05& 0.34\tabularnewline
\midrule
\multirow{4}{*}{\textcite{bowmanTestingMonotonicityRegression1998}}&m1& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&m2& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&m3& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.9& 1.0& 1.0\tabularnewline
&m4& 0.0& 0.0& 0.0& 0.01& 0.02& 0.0& 0.34& 0.33& 0.28\tabularnewline
\midrule
\multirow{4}{*}{MDCS}&m1& 0.03& 0.02& 0.02& 0.0& 0.01& 0.0& 0.0& 0.0& 0.0\tabularnewline
&m2& 0.98& 0.99& 0.95& 1.0& 1.0& 0.94& 0.18& 0.35& 0.65\tabularnewline
&m3& 0.89& 0.93& 1.0& 0.9& 0.97& 0.99& 0.16& 0.22& 0.29\tabularnewline
&m4& 0.89& 0.91& 0.94& 0.88& 0.92& 0.99& 0.51& 0.68& 0.81\tabularnewline
\midrule
\multirow{4}{*}{MDSS}&m1& 0.05& 0.07& 0.04& 0.06& 0.04& 0.03& 0.05& 0.07& 0.05\tabularnewline
&m2& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.79& 0.96& 1.0\tabularnewline
&m3& 1.0& 1.0& 1.0& 1.0& 1.0& 1.0& 0.67& 0.83& 0.97\tabularnewline
&m4& 0.98& 1.0& 1.0& 0.99& 1.0& 1.0& 0.84& 0.99& 1.0\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_test/res_mono_test_mono_sup.tex <==
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{curve}&\multicolumn{3}{c}{$\sigma = 0.001$}&\multicolumn{3}{c}{$\sigma = 0.01$}&\multicolumn{3}{c}{$\sigma = 0.1$}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
&&n = 50&100&200&n = 50&100&200&n = 50&100&200\tabularnewline
\midrule
\midrule
\multirow{5}{*}{MD (CS) sup}&$x$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.01& 0.0& 0.0\tabularnewline
&$x^3$& 0.01& 0.0& 0.0& 0.02& 0.02& 0.01& 0.02& 0.0& 0.01\tabularnewline
&$x^{1/3}$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.02& 0.0& 0.0\tabularnewline
&$e^x$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&$1/(1+e^{-x})$& 0.0& 0.0& 0.0& 0.01& 0.0& 0.0& 0.01& 0.0& 0.0\tabularnewline
\midrule
\multirow{5}{*}{MD (CS)}&$x$& 0.02& 0.02& 0.04& 0.04& 0.04& 0.05& 0.03& 0.08& 0.06\tabularnewline
&$x^3$& 0.04& 0.03& 0.0& 0.06& 0.03& 0.06& 0.06& 0.07& 0.08\tabularnewline
&$x^{1/3}$& 0.03& 0.04& 0.07& 0.02& 0.02& 0.05& 0.08& 0.06& 0.06\tabularnewline
&$e^x$& 0.04& 0.03& 0.02& 0.01& 0.02& 0.01& 0.1& 0.05& 0.09\tabularnewline
&$1/(1+e^{-x})$& 0.02& 0.05& 0.02& 0.03& 0.07& 0.05& 0.02& 0.02& 0.02\tabularnewline
\midrule
\multirow{5}{*}{MD (SS) sup}&$x$& 0.02& 0.0& 0.0& 0.08& 0.0& 0.0& 0.06& 0.0& 0.0\tabularnewline
&$x^3$& 0.07& 0.0& 0.0& 0.08& 0.0& 0.0& 0.02& 0.0& 0.0\tabularnewline
&$x^{1/3}$& 0.06& 0.0& 0.0& 0.08& 0.0& 0.0& 0.08& 0.0& 0.01\tabularnewline
&$e^x$& 0.01& 0.0& 0.0& 0.03& 0.0& 0.0& 0.06& 0.0& 0.0\tabularnewline
&$1/(1+e^{-x})$& 0.03& 0.0& 0.0& 0.11& 0.0& 0.0& 0.04& 0.0& 0.0\tabularnewline
\midrule
\multirow{5}{*}{MD (SS)}&$x$& 0.12& 0.09& 0.06& 0.17& 0.07& 0.1& 0.12& 0.03& 0.05\tabularnewline
&$x^3$& 0.1& 0.01& 0.02& 0.11& 0.02& 0.01& 0.05& 0.02& 0.02\tabularnewline
&$x^{1/3}$& 0.15& 0.02& 0.02& 0.13& 0.01& 0.04& 0.11& 0.03& 0.02\tabularnewline
&$e^x$& 0.11& 0.05& 0.05& 0.15& 0.06& 0.11& 0.12& 0.01& 0.07\tabularnewline
&$1/(1+e^{-x})$& 0.14& 0.12& 0.15& 0.23& 0.04& 0.02& 0.05& 0.03& 0.01\tabularnewline
\midrule
\multirow{5}{*}{Meyer}&$x$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&$x^3$& 0.52& 0.75& 1.0& 0.09& 0.04& 0.09& 0.02& 0.04& 0.05\tabularnewline
&$x^{1/3}$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.05& 0.05& 0.03\tabularnewline
&$e^x$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.01& 0.0& 0.0\tabularnewline
&$1/(1+e^{-x})$& 0.0& 0.0& 0.0& 0.01& 0.0& 0.0& 0.07& 0.08& 0.02\tabularnewline
\midrule
\multirow{5}{*}{Ghosal}&$x$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&$x^3$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&$x^{1/3}$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&$e^x$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
&$1/(1+e^{-x})$& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0& 0.0\tabularnewline
\midrule
\multirow{5}{*}{Bowman}&$x$& 0.0& 0.0& 0.0& 0.1& 0.01& 0.0& 0.02& 0.0& 0.01\tabularnewline
&$x^3$& 0.0& 0.0& 0.0& 0.13& 0.14& 0.21& 0.21& 0.19& 0.2\tabularnewline
&$x^{1/3}$& 0.01& 0.0& 0.0& 0.01& 0.0& 0.0& 0.02& 0.01& 0.04\tabularnewline
&$e^x$& 0.0& 0.0& 0.0& 0.06& 0.0& 0.0& 0.06& 0.0& 0.0\tabularnewline
&$1/(1+e^{-x})$& 0.14& 0.0& 0.0& 0.05& 0.01& 0.03& 0.0& 0.02& 0.01\tabularnewline
\bottomrule
\end{tabular}

